Hierarchical Knowledge Graphs: A Novel Information Representation for Exploratory Search Tasks

In exploratory search tasks, alongside information retrieval, information representation is an important factor in sensemaking. In this paper, we explore a multi-layer extension to knowledge graphs, hierarchical knowledge graphs (HKGs), that combines hierarchical and network visualizations into a unified data representation asa tool to support exploratory search. We describe our algorithm to construct these visualizations, analyze interaction logs to quantitatively demonstrate performance parity with networks and performance advantages over hierarchies, and synthesize data from interaction logs, interviews, and thinkalouds on a testbed data set to demonstrate the utility of the unified hierarchy+network structure in our HKGs. Alongside the above study, we perform an additional mixed methods analysis of the effect of precision and recall on the performance of hierarchical knowledge graphs for two different exploratory search tasks. While the quantitative data shows a limited effect of precision and recall on user performance and user effort, qualitative data combined with post-hoc statistical analysis provides evidence that the type of exploratory search task (e.g., learning versus investigating) can be impacted by precision and recall. Furthermore, our qualitative analyses find that users are unable to perceive differences in the quality of extracted information. We discuss the implications of our results and analyze other factors that more significantly impact exploratory search performance in our experimental tasks.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> sec.Framework.tex <==
\section{Evaluation Framework}

\el{Changed my mind; I think this should be its own section now. But I'm starting to think it should come after the SIGIR paper. I'm not going to go any further here until we decide ...}\\
% \bs{I understand the point of having the Framework here if we are able to do a good job of refining it to reflect an overall plan for the entire paper. That is, System Support for ES section that indicates any ES support system needs two components: extraction and representation. Then specify the plan for separation of automatic extraction challenges (i.e. presence of errors) from evaluating representations in terms of their structure and whether and how they are effective in support ES tasks. So this section can be kept at the beginning of the paper as a roadmap for the rest of the paper or be placed After Part 1 to facilitate transition to Part 2. Thoughts?}

In order to evaluate how varying levels of precision and recall in IE impact user behavior, it is necessary to embed the IE algorithm in a system that supports the overall task. As we noted earlier, in this paper, our primary interest is in how varied levels of precision and recall in IE impact exploratory search.


With this goal in mind, in this section we describe a framework for evaluating systems that support exploratory search.  We first focus on the necessary system components to support exploratory search, including an IE algorithm and an interface that leverages IE output to support user interaction. \textcolor{red}{We then characterize the behavior of our IE algorithm to demonstrate that our system includes varied levels of precision and recall.}

\subsection{System Support for Exploratory Search}
As noted in the introduction, to support exploratory search, a system must have two components: an information extraction system that can identify and extract relevant information from a corpus (e.g., search engine results); and, an interactive UI that presents the information to users and allows users to browse the extracted information for sensemaking~\cite{jul97, olston03}.
% \begin{enumerate}
%     \item An Open IE system that can extract information from a set of retrieved documents (i.e. search results) and present that information.
%     \item An Interactive Search UI that enables users to effectively explore and make sense of the retrieved information by providing meaningful representations and visualizations of this information.
% \end{enumerate}
Any arbitrary system designed to support exploratory search will exist on a range from a standard search engine interface (an ordered list where a user can select and browse individual documents) to systems that extract and synthesize information for the user. An example of the latter type of system include those found at the TREC Complex Answer Retrieval track~\cite{dietz17trec} which explores the design of systems that apply information extraction to synthesize content and generate an essay on a particular topic. Ultimately, any system on this spectrum requires the two components identified above: an information extraction component and an interactive UI to support browsing.
% Given the above two components, any system can span a range of behaviors. For example, a search engine interface provides some support for exploratory search by retrieving documents, presenting documents as an ordered list, and allowing users to browse the document collection by reading individual documents to identify and synthesize information.  At the other extreme, information retrieval researchers examine techniques including automatic document summarization and other forms of information synthesis to more directly support exploratory search.  As one example of this extreme, the CAR track in TREC \cite{dietz17trec} explores how effectively information extraction systems can be used to synthesize content and generate an essay on a topic of interest.

A common approach to present-day exploratory search systems is to leverage IE to identify relevant entities and their relationships within the retrieved documents. These entities and relationships can then be displayed in graphical form (e.g., as a knowledge graph, or hierarchy, or concept map, etc) which provides the user with a spatial representation of the information space for sensemaking~\cite{pirolli2000}. This representation can then be embedded in an interface that allows a user to interact with the representation, to filter and select specific content, and essentially to explore the information returned~\cite{sarrafzadeh16}. 
% As  a  result, the underlying representation is  linked  to  the interface  that  contains  it  and  supports  manipulation  and exploration of it~\cite{hearst06}.


% Open Information Extraction (Open IE) was originally formulated as a function from a document to a set of tuples indicating a semantic relation between a predicate phrase and its arguments \cite{banko07}, and was later refined as 
% generating a structured representation of information in text, usually in the form of triples or n-ary propositions without relying on any pre-defined ontology schema. Since its introduction, Open IE has gained substantial and consistent attention and many automatic extractors were created (see \cite{cui18, niklaus2018survey} for a survey of these systems). Given that Open IE systems are mostly used as a component within larger frameworks \cite{stanovsky16, chu07, christensen13, balasubramanian13}, their output quality can greatly impact the overall performance of the target application they are utilized for.

% User interaction with search interfaces differs depending on the type of task, the
% amount of time and effort available to invest in the process, and the domain
% expertise of the information seeker \cite{hearst09}.  The simple interaction dialogue used in Web search engines is most appropriate for finding answers to questions or to finding Web sites or other resources that act as search starting points.  
%But, as Marchionini [89] notes, the ``turn-taking'' interface of Web search engines is inherently limited and is many cases is being supplanted by speciality search engines – such as for travel and health information – that offer richer interaction models.



% Marchionini notes that there are interactive aspects to exploratory search, rather than simply viewing the query satisfaction or information retrieval problem as optimally matching documents to a query. Characteristics of these interfaces, drawn from research in human-computer interaction, include the use of high-level overviews and rapid previews to facilitate sensemaking during the exploratory process. The incorporation of overviews argues for some organization of search results that both presents this overview and allows the user to explore the data and its interconnected relationships more fully through filtering and the examination of user-selected details \cite{shneiderman96}.

\subsection{Evaluating Exploratory Search Systems}

\textcolor{red}{Given that our goal is to understand how errors in extraction can impact exploratory search tasks, it is necessary to analyze IE algorithms as a component within larger frameworks~\cite{stanovsky16, chu07, christensen13, balasubramanian13}.} There are two aspects to system performance: accuracy and effectiveness. % Accordingly, we require a mechanism to assess the accuracy of extraction. 
Assessing the accuracy of an algorithm can be performed through benchmarking and/or combined efforts tasks (e.g., TREC or CLEF tasks). System effectiveness for exploratory search, on the other hand, requires evaluating how well the systems aids in the exploratory search tasks it is designed around. In the following two subsections, we describe in more detail, these two types of assessments.  Our goal can therefore be stated as an attempt to characterize the impact of accuracy on effectiveness.

% Given a system to support exploratory search, a related question is how best to characterize the effectiveness of an exploratory search system.  There are two aspects to system performance: accuracy and effectiveness.  To assess system accuracy, a benchmark is needed to evaluate the accuracy of the extracted content.  Furthermore, to assess system effectiveness, we must assess how well the system aids in the exploratory search task.  To accomplish this, a set of exploratory search tasks that elicit exploratory search style information seeking.

\subsubsection{System Accuracy}
Evaluating information extraction is challenging.  There are no clear guidelines as to what constitutes a valid proposition to be extracted, and most information extraction evaluations  consist of a post-hoc manual evaluation of a small output sample~\cite{stanovsky16}.  There is also no agreement on an appropriate data set to use for information extraction
% Moreover, none of the datasets used for assessing the performance of different systems is widely agreed upon 
~\cite{niklaus2018survey}.
However, Stanovsky and Dagan \cite{stanovsky16} have developed a methodology that leveraged the recent formulation of QA-SRL~\cite{he05} to create the first independent and large-scale gold benchmark corpus.\footnote{The corpus is available at: https://github.com/gabrielStanovsky/oie-benchmark} Stanovsky and Dagan's benchmark is based on a set of guiding principles that underlie most Open IE approaches. This benchmark has provided an opportunity to evaluate the output of an Open IE system using both precision and recall.  While acknowledging that this benchmark may not be perfect, we leverage it as the most up-to-date standard for evaluating IE systems.
% Given that, to the best of our knowledge, this is the most up-to-date and recent such benchmark but we also note that task specific benchmarks may also be necessary in the future to meet shifting demands on downstream systems. 
% In order to address aforementioned difficulties,  Stanovsky and Dagan (2016) recently made a first attempt in standardizing the Open IE evaluation by providing a large gold benchmark corpus. 
% It is based on a set of consensual guiding principles that underlie most Open IE approaches. 
% Those principles cover the core aspects of the task of Open IE, allowing for a clearer formulation of the problem to be solved. 
% The three key features to consider are the following: Assertedness, Minimal Propositions and Completeness and Open Lexicon.



\subsubsection{System Effectiveness}
It has long been understood in IR that a system understanding of relevance is not always consistent with what a user desires~\cite{saracevic} and so we must also understand how systems impact user performance.  To do this, representative search tasks are required. Marchionini~\cite{marchionini06}, referencing Bloom's taxonomy of educational objectives~\cite{bloom56}, distinguishes three broad categories of search tasks as {\it Lookup}, {\it Learn}, and {\it Investigate}. While these categories are depicted as overlapping activities, exploratory search is more pertinent to the {\it Learn} and {\it Investigate} activities.  As a result,  exploratory search is defined as searching that supports learning, investigating, comparison or discovery~\cite{kules08, white09}. 
From this understanding, we can distill exploratory search tasks into fitting into one of two themes. 
The first theme includes those tasks that facilitate learning to achieve knowledge acquisition, comprehension of concepts, interpretation of ideas and comparison or aggregation of concepts. The second theme covers those investigative tasks that involve discovery, analysis, synthesis and evaluation. 

% Li and Belkin \cite{li_belkin08} extensively reviewed existing classifications of tasks and identified essential facets and attributes of different types of tasks ranging from work tasks to information related tasks. The proposed classification includes Generic facets of tasks (Source of task, Task doer, Time, Product, Process and Goal) and Common attributes of task (Task characteristics and User's perception of tasks).

Based upon the aforementioned works and a survey of existing classification by Li and Belkin~\cite{li_belkin08}, we believe that exploratory search tasks should: provide uncertainty and ambiguity about the information need and in how to satisfy it; suggest a specific knowledge acquisition, comparison or discovery task; be in an unfamiliar domain for the searcher; represent a situation that a user can relate to and identify with; be of sufficient interest to test users; and, be formulated such that the user has enough imaginative context to facilitate immersion in the task. Any task that meets these criteria provides sufficient complexity that the end-to-end experience with an exploratory search system can be fully and properly assessed.

% This  brief  review  suggests  that  exploratory  search 
% tasks should: 
% \begin{itemize}
%     \item Indicate uncertainty, ambiguity in information need and/or need for discovery. 
%     \item Suggest a knowledge acquisition, comparison, or 
% discovery task 
%     \item Be an unfamiliar domain for the searcher
%     \item Provide a low level of specificity about:\\ 
% - The information necessary for their search\\ 
% - How to find the required information\\  
% - How to recognize the required information\\
%     \item Be a situation which the test persons can relate to and in which they can identify themselves  
%     \item Be a situation that the test persons find topically interesting 
%     \item Be a situation that provides enough imaginative context  in order for the test persons to be able to relate and apply the situation. 
% \end{itemize}









% In order to design a framework to be able to investigate the effect of errors in the output of IE systems on exploratory search outcomes we can envision the following components:
% \begin{enumerate}
%     \item An Open IE system that can extract information from a set of retrieved documents (i.e. search results) and present them as entity-relationship tuples.
%     \item A benchmark to evaluate the accuracy of the extracted tuples as well as providing gold standard extractions to indicate an upper bound for search performance.
%     \item An Interactive Search UI that enables users to effectively explore and make sense of the retrieved information by providing meaningful representations and visualizations of this information.
%     \item A set of exploratory search tasks that provide a genuine information need and motivate searchers to engage in information seeking activities that can elicit exploratory behavior. 
%     \item A controlled experimental design that allows a reasonable assessment of efficacy of these information representations at different levels of accuracy in supporting users' exploratory information seeking goals.
% \end{enumerate}

% The following subsections elaborate on each of these components.

% \subsection{Information Extraction}
% Open Information Extraction (Open IE) was originally formulated as a function from a document to a set of tuples indicating a semantic relation between a predicate phrase and its arguments \cite{banko07}, and was later refined as 
% generating a structured representation of information in text, usually in the form of triples or n-ary propositions without relying on any pre-defined ontology schema. Since its introduction, Open IE has gained substantial and consistent attention and many automatic extractors were created (see \cite{cui18, niklaus2018survey} for a survey of these systems). Given that Open IE systems are mostly used as a component within larger frameworks \cite{stanovsky16, chu07, christensen13, balasubramanian13}, their output quality can greatly impact the overall performance of the target application they are utilized for.

% \subsection{Benchmark for Evaluation}
% Despite the widespread use of Open IE systems in various downstream applications, there are no clear guidelines as to what constitutes a valid proposition to be extracted, and most OpenIE evaluations usually consist of a post-hoc manual evaluation of a small output sample \cite{stanovsky16}.
% Moreover, none of the datasets that were used for assessing the performance of different systems is widely agreed upon \cite{niklaus2018survey}. 
% More recently, Stanovsky and Dagan \cite{stanovsky16} developed a methodology that leveraged the recent formulation of QA-SRL \cite{he05} to create a first independent and large scale gold benchmark corpus \footnote{The corpus is available at: https://github.com/gabrielStanovsky/oie-benchmark}.
% % In order to address aforementioned difficulties,  Stanovsky and Dagan (2016) recently made a first attempt in standardizing the Open IE evaluation by providing a large gold benchmark corpus. 
% It is based on a set of consensual guiding principles that underly most Open IE approaches proposed so far, as they have identified.  Those principles cover the core aspects of the task of Open IE, allowing for a clearer formulation of the problem to be solved. The three key features to consider are the following: Assertedness, Minimal Propositions and Completeness and Open Lexicon.
% This benchmark has provided an opportunity to evaluate the output of an Open IE system using both precision and recall oriented metrics as well as an objective and unified way to evaluate and compare prominent Open IE systems.

% % Though a multitude of systems for Open IE have been developed over the last decade, a clear formal specification of what constitutes a valid relational tuple is still missing.   This lack of a well-defined, generally accepted task definition prevented the creation of an established, large-scale annotated corpus serving as a gold standard dataset for an objective and reproducible cross-system comparison.   As a consequence, to date, Open IE systems were predominantly evaluated by hand on small-scale corpora that consist of only a few hundred sentences, thereby ignoring one of the fundamental goals of Open IE: scalability to large amounts of text.  Moreover, none of the datasets that were used for assessing the performance of different systems is widely agreed upon.
% %  Besides, although Open IE methods are targeted at being domain independent and able to cope with heterogeneous datasets, the corpora used in the evaluation process are restricted to the news, Wikipedia and Web domains for the most part.  Accordingly, no clear statement about the portability of the approaches to various genres of text is possible. In addition, most evaluation procedures described in the literature focus on precision-oriented metrics, while either completely ignoring recall or using some kind of proxy, such as yield, i.e.  the total number of extractions labeled as correct, or coverage, i.e.  the percentage of text from the input that is contained in at least one of the extractions.  Hence, the absence of a standard evaluation procedure makes it hard to replicate and compare the performance of different Open IE systems.

% % In order to address aforementioned difficulties,  Stanovsky and Dagan (2016) recently made a first attempt in standardizing the Open IE evaluation by providing a large gold benchmark corpus. It is based on a set of consensual guiding principles that underly most Open IE approaches proposed so far, as they have identified.  Those principles cover the core aspects of the task of Open IE, allowing for a clearer formulation of the problem to be solved. The three key features to consider are the following: Assertedness, Minimal Propositions and Completeness and Open Lexicon.
% \subsection{Exploratory Search Interface}
% User interaction with search interfaces differs depending on the type of task, the
% amount of time and effort available to invest in the process, and the domain
% expertise of the information seeker \cite{hearst09}.  The simple interaction dialogue used in Web search engines is most appropriate for finding answers to questions or to finding Web sites or other resources that act as search starting points.  
% %But, as Marchionini [89] notes, the ``turn-taking'' interface of Web search engines is inherently limited and is many cases is being supplanted by speciality search engines – such as for travel and health information – that offer richer interaction models.

% One challenge with any interface that presents search results from an exploratory query to users is that the goal is rarely a static representation of the content returned by a user's query.  Instead, the goal is to develop an interface that allows a user to interact with the content, to filter and select specific content, essentially to explore the information returned \cite{sarrafzadeh16}.   As  a  result,  the  representation  is  linked  to  the interface  that  contains  it  and  supports  manipulation  and exploration of it \cite{hearst06}.

% Marchionini notes that there are interactive aspects to exploratory search, rather than simply viewing the query satisfaction or information retrieval problem as optimally matching documents to a query. Characteristics of these interfaces, drawn from research in human-computer interaction, include the use of high-level overviews and rapid previews to facilitate sensemaking during the exploratory process. The incorporation of overviews argues for some organization of search results that both presents this overview and allows the user to explore the data and its interconnected relationships more fully through filtering and the examination of user-selected details \cite{shneiderman96}.

% Within this space some past work has explored the efficacy of different knowledge representations \cite{novick01} and how competing representations fare in presenting results for exploratory search tasks (e.g. \cite{norman88, capra07, sarrafzadeh14, amadieu14, sarrafzadeh16}).
% %While some past research has explored using questionnaires to determine the efficacy of different knowledge representations [30], or has evaluated the efficacy of hierarchies, networks, or concept maps with respect to ordered lists (e.g. [1, 9, 10, 27, 38]
% %\cite{capra07, norman88, %ducheneaut01, sarrafzadeh14, amadieu10, %amadieu14, carnot03}


% \subsection{Exploratory Search Tasks}
% In order to effectively evaluate interactive IR systems, it will be necessary to develop more complex search tasks and more exploratory search tasks.
% Designing exploratory search tasks is an important but challenging requirement for successfully evaluating exploratory search interfaces. 
% %When creating any type of search task, there is a challenge of creating a realistic, representative task. When creating exploratory search tasks, there is an additional burden of actually inducing an exploratory search \cite{kules08}.
% As Kules and Capra \cite{kules08} have pointed out, ``designing tasks for studies of exploratory search can be especially difficult due to the goal of inducing an exploratory (rather than directed) style search, wherein searchers will individually interpret the tasks, their relevance, and the results \cite{kules08shneiderman} - while maintaining some level of experimental control''.
% % This high level goal of doing an exploratory search drives how users interpret their tasks, their relevance and their results \cite{kules08shneiderman}.

% As well, given that search tasks can vary among many dimensions (e.g. their complexity, structure and granularity), we need to be able to construct tasks having particular attributes, knowing that our study findings can then be generalized to all search tasks having those attributes \cite{wildemuth12}.

% Since Marchionini's seminal work on classifying different types of search tasks \cite{marchionini06}, exploratory search is defined as searching that supports learning, investigating, comparison or discovery \cite{kules08, white09}. 

% Past research has identified different attributes of search tasks that elicit different information seeking behaviors. Marchionini, referencing Bloom's taxonomy of educational objectives \cite{bloom56}, distinguishes three broad categories of search tasks as Lookup, Learn and Investigate. While these categories are depicted as overlapping activities, exploratory search is more pertinent to the learn and investigate activities.

% Searches that support learning aim to achieve knowledge acquisition, comprehension of concepts, interpretation of ideas and comparison or aggregation of concepts. On the other hand, Investigate category is positioned at the highest level of Bloom's taxonomy of objectives and involves discovery, analysis, synthesis and evaluation. 

% Li and Belkin \cite{li_belkin08} extensively reviewed existing classifications of tasks and identified essential facets and attributes of different types of tasks ranging from work tasks to information related tasks. The proposed classification includes Generic facets of tasks (Source of task, Task doer, Time, Product, Process and Goal) and Common attributes of task (Task characteristics and User's perception of tasks).

% This  brief  review  suggests  that  exploratory  search 
% tasks should: 
% \begin{itemize}
%     \item Indicate uncertainty, ambiguity in information need and/or need for discovery. 
%     \item Suggest a knowledge acquisition, comparison, or 
% discovery task 
%     \item Be an unfamiliar domain for the searcher
%     \item Provide a low level of specificity about:\\ 
% - The information necessary for their search\\ 
% - How to find the required information\\  
% - How to recognize the required information\\
%     \item Be a situation which the test persons can relate to and in which they can identify themselves  
%     \item Be a situation that the test persons find topically interesting 
%     \item Be a situation that provides enough imaginative context  in order for the test persons to be able to relate and apply the situation. 
% \end{itemize}

% Wildemuth and Freund \cite{wildemuth12} also identify:

% Exploratory search tasks are associated with the goals of learning and/or
% investigation In Marchionini's seminal [ 35 ] paper on exploratory search, he depicted exploratory search processes as involving two major types of search activities: learning and investigation. White and Roth [ 50 ] , in their recent review of exploratory search, also preserved this perspective, expanding it slightly to argue that learning ``is not only about knowledge acquisition, but rather the development of higher-level intellectual capabilities within a particular subject area'' [ 50 , p.13] . Similarly, Vakkari [ 46 ] maintained the link to both learning and investigative search goals. He suggested that investigative search is invoked ``when actors are exploring possible conceptualizations of their topic'' [46 , p.3 ] , and that learning is illustrated by the increase in the exhaustivity and specificity of the searcher's mental model of the topic as the search progresses.




==> sec.Introduction.tex <==
\section{Old Introduction}
Information Retrieval (IR) research explores a wide range of questions connected to the goal of helping a user find useful information in response to a need \cite{Allan05}. Given this goal and the availability of on-line information, it is unsurprising that significant IR research effort exists in supporting web search \cite{broder2002,  marchionini06, wilson10, white09}.  It is well-established that, within the domain of web search, there exists two broad categories of search: look-up searches, which leverage a ``search by query'' strategy for information seeking%\cite{athukorala16}
; and browsing (i.e., ``search by navigation'') \cite{olston03,jul97}. Our interest is primarily in the second category of information seeking, and, in particular, in the broad category of information seeking that has been classified as \emph{Exploratory Search}~\cite{marchionini06}.
% The Web has provided the opportunity to browse and navigate through an extensive information space. However, beyond simply finding basic answers, web searchers also engage in learning and discovery. Search activities are commonly divided into two broad categories: lookup and exploratory \cite{marchionini06}. The predominant design goal in IR systems has been fast and accurate completion of lookup searches \cite{athukorala16}, that are following a ``search by query'' paradigm.
% Although there has been a lot of research on understanding exploratory search (see White and Roth \cite{white09} for a survey), there are many open questions when it comes to the design of IR systems that provide tailored and adaptive support.

The 2018 SWIRL Workshop \cite{swirl2018} emphasizes the need for continuing and ongoing research in supporting complex, evolving and exploratory information seeking goals, which requires advances in the algorithms to provide information, the interfaces that represent this information, and the evaluation methods that support these goals. 
Prior work indicates that interfaces supporting exploratory search benefit from both ``search by query'' and ``search by navigation'' paradigms~\cite{olston03,jul97},
and that such interfaces require concise and understandable representations of search results that accommodate a searcher's `state of knowledge' and provide `information scent' to guide the user during navigation \cite{hearst09, pirolli2000, olston03, sarrafzadeh16, sarrafzadeh17}.
 
While representing information is critical to effective support of exploratory search, the process of extracting and presenting that information to the user is challenging. Information extraction (IE) algorithms are not perfect \cite{stanovsky16}, meaning that the base level information to be presented to a user may contain errors and omissions, and, as such, may reflect compromises in either \emph{precision} or \emph{recall} by the algorithm. The TAC~\footnote{https://tac.nist.gov/} and TREC~\footnote{https://trec.nist.gov/} tracks on evaluating IE and question answering (QA) algorithms report varying levels of precision and recall for these algorithms when compared against manually created ground truth datasets. 

While boosting the precision and/or recall of information extraction systems is valuable, it is unclear whether IE algorithms will attain human-like accuracy in the near term. Accordingly, given that IE algorithms are not perfect, how do current precision and recall levels in IE algorithms impact user performance in exploratory search tasks?  

% we wish to investigate is the effect of errors on exploratory search tasks. In particular, if we assume that the goal of exploratory search is to develop knowledge and that how retrieved data is presented and interacting with this data via browsing are crucial aspects of such search, we seek to determine the impact these presentations have on this development of knowledge when the data being examined is produced by a system with impaired precision or recall.

There are three primary reasons that we feel the above is an open and significant question in information retrieval. First, in the document retrieval community, assessments of human performance in question answering tasks given varied precision and recall has produced mixed results, with some assessments finding that information retrieval precision and recall can significantly impact human performance \cite{smucker10, sanderson10} and others finding no significant impact \cite{hersh2000, hersh02, turpin06, smith08}.  Second, if, in exploratory search tasks, there is a need to support both query and browsing~\cite{olston03,jul97}, there is some evidence that interaction with search results (i.e., browsing) may limit the negative impacts of compromised precision and recall~\cite{lin08, vakkari12}.  Finally, while it would seem obvious that the goal of boosting precision and recall is primarily to satisfy user requirements with respect to IE -- is the IE algorithm accurate enough for the user's task? --
%we note that IE is a necessary pre-cursor to creating representations of information content \cite{pirolli2000} and that state-of-the-art IE algorithms are limited in precision and recall \cite{stanovsky16}.  However, 
we have found only one examination of how error-prone IE impacts user performance \cite{chu07}, and the goal of this earlier evaluation was to assess the impact on document retrieval, not on exploratory search.

In this paper, we present a mixed-methods study \cite{creswell2013research} that examines the impact of imperfect IE on exploratory search tasks.  To conduct this evaluation, we leverage an existing system that supports exploratory search tasks via hierarchical knowledge graphs (HKGs) \cite{sarrafzadeh17}.  Users interact with two HKGs, one created manually by human experts (the typical approach to generating ground truth to benchmark IE systems \cite{stanovsky16}) and a second graph that was automatically generated and exhibits significantly lower precision and recall compared to the manually generated graph.  
% We benchmark the automatic IE algorithm, and show that it exhibits significantly lower precision and recall of entity-relationship tuples than manually extracted entity-relationship tuples, yielding two data points with substantial differences in precision and recall.

While our expectation was that precision and recall would impact user performance (i.e., success in an exploratory search task) or the effort expended during search (e.g., the number of documents viewed), our results indicate that neither performance nor effort was significantly impacted by differing levels of precision and recall. To probe this result in greater detail, we analyze qualitative data collected via observations and interviews.  Our qualitative data indicates that task characteristics may be an important factor to consider in exploratory search.  Specifically, for investigate-style tasks \cite{marchionini06} where there is a defined set of facts to retrieve, recall may impact user behavior because it is necessary to find specific facts within the information presented.  In contrast, more open-ended synthesis or comparison tasks, where salient data can be more flexibly applied by the user, seem more resilient to lower recall rates.  
%We perform follow-on quantitative analysis that further triangulates with these results from qualitative observations.  We conclude by discussing the implications for systems designed to support exploratory search.

Overall, this paper makes two contributions to IE. First, it demonstrates an approach to evaluating IE that embeds IE in a task flow and evaluates IE performance in situ using a balanced mix of quantitative and qualitative (i.e., mixed) methods. While the approach to in situ IE evaluation is straight forward and both qualitative and quantitative analyses are mature research methods, we argue that this in situ evaluation is essential in ensuring that improvements in IE performance are meaningful. In particular, if one accepts that the goal of improved IE is to substantively improve task outcomes, then the fact that we have found only one instance of IE evaluation that considers user performance \cite{chu07} is a significant concern, one that this paper provides a roadmap for addressing in future work. Second, through our quantitative and, in particular, our qualitative results, this paper highlights how different exploratory search task types (e.g., investigate vs compare/synthesize) may be more or less resilient to varied precision and recall. Understanding this is a first step toward addressing the contradictory effects that variations in precision and recall have had on information retrieval outcomes when those outcomes are measured via human performance metrics~\cite{hersh2000, hersh02, lin08, turpin06, smith08, smucker10, sanderson10, vakkari12}.
\vspace{-1mm}

% Leave this for RW.  \fixme{Our results are highly significant.  We were able to identify only one examination, by Chu-Carrol and Prager \cite{chu07}, on how search performance degrades in the face of imperfect named entity and relation extraction. Their experimental results demonstrated that significant document retrieval gain can be achieved when state-of-the-art IE systems are used and that recall has more significant impact on document retrieval performance than precision when adopting the MAP metric.}

% Doesn't feel right here. It is expected that algorithm performance in precision and recall would impact information seeking behaviours; however one thing that we do know from past research in IR is that it is difficult to determine the impact of recall and precision on human performance in search tasks. In the Document Retrieval community, the effect of human performance in question/answering tasks given varied precision and recall has been mixed, with some assessments finding that precision and recall significantly impacts human performance and others finding no significant impact.

%More recently, the recognition that there is more to information seeking activities than look-up search has led to many extensions and alternatives to the standard ``document retrieval paradigm''. These extensions aimed at supporting users by providing ``information'' and not documents and also involving users more actively in the search process.
%A dominant technique towards automatic retrieval of information is Information Extraction (IE). IE aims at (semi)automatic collection of triples from textual corpora of a given domain (e.g., <Napoleon, invaded, Russia> is extracted from “Napoleon invaded Russia.”). These triples indicate the relationship between two entities. 

% To elaborate, within the domain of exploratory search researchers have pointed to the need for representation and interaction with those representations, as an important component that allows users to see, comprehend and acquire knowledge.
% In fact, the main challenge with supporting exploratory search is that the process of extracting and then representing that information is challenging. From the perspective of the representation it's difficult to know how best to represent information to users so that they can see, comprehend and interact with content.\\
% \textcolor{red}{ - there has been some recent work in the IR community that is addressing this [cite].}\\

% Similarly Open Information Extraction (Open IE) \cite{banko07}, as a dominant technique towards automatic extraction of information from documents, is kind of assumed to be present within this domain. But IE has its own challenges associated with it, in particular IE algorithms are complex, frequently error prone and suffer from problems of variable precision and recall [cite some IE papers].

% % And researchers are only beginning to explore the effect of IE errors on various aspects of Information Retrieval. --> 
% Despite the core need for Information Extraction as a component of the exploratory search, we have identified very limited work exploring specifically the effects of IE errors in the IR domain. And none of that work has looked at IE errors and its effect of comprehension and interaction with representations in the domain of exploratory search.

% More broadly in IR there is an interest in errors and their effect on different aspects of information retrieval. First, a number of studies have investigated whether variation in relevance judgment exist and how they affect measures of retrieval performance [References]. The overall conclusion was that there are indeed significant variations in relevance assessments among judges, however, IR systems evaluation and ranking were generally robust to these variations \cite{voorhees2000, bailey08}. As well, many researchers have challenged the Cranfield approach to system evaluation, and whether there a relationship between system and user effectiveness.
% %maintaining that real world search is more complex and that system efficacy cannot be accurately assessed with such studies. These authors point out that relevance is not a fixed notion \cite{meadow85}, interaction is the key element of successful retrieval system use \cite{swanson77} and relevance based measures do not capture the complete picture of user performance.  
% Studies exploring to which extent human retrieval effectiveness varies with system effectiveness have resulted in contradictory findings. 
% Earlier studies have demonstrated that improved system effectiveness does not translate into a benefit for users.
% %For example in Document Retrieval and Relevance Judgement Community researchers have explored how errors affect information retrieval tasks. And in particular how errors affect human performance. 

% Unfortunately all of this work is conflicted and there are multiple perspectives on the cost of errors, ``varying from insignificant to highly significant'', in terms of how it affects human performance.\\
% \textcolor{red}{ -- reasons for these conflicts ...}\\

% One thing that we do know that affects errors vis-a-vis human performance is the ability to interact with the search results [cite Mark] 

% In this paper we are looking specifically at knowledge representations for exploratory search 
% % and how one recent knowledge representation for exploratory search, hierarchical knowledge graphs, 
% and how IE errors which result in precision and recall problems in the underlying dataset affect knowledge acquisition / information seeking behaviors.









==> sec.OriginalQualitative.tex <==
\section{Qualitative Findings}
The qualitative analysis of our post task interviews resulted in a rich characterization of the two exploratory search tasks and how they compare with respect to their perceived complexity as well as main distinguishing attributes. We found that our participants were split in their perception of the complexity of these two tasks and that a variety of factors such as prior knowledge of the searcher, interpretation of the task, and the strategies employed impacted their perception. 

Participants who found the History task more difficult ([P1-5, P7, P9, P10, P15, P20]) mentioned a variety of reasons including \textit{representation does not match the perceived domain structure} [P3, P10, P15], \textit{Politics is a more familiar domain} [P5, P7, P10], \textit{``needed a deeper exploration''} [P9], \textit{``searching without a keyword''}[P3], \textit{``more detailed fact finding''}[P6, P8, P13].

A different group of participants, however, perceived the Politics tasks to be more difficult [P4, P6, P11-13, P17-18, P21-22, P24-25]. The most common rationales included \textit{``Politics task asks a higher level question and needs a higher level understanding of a domain''} [P8, P10], \textit{``involves learning, complex reasoning and interpretation''} [P6, P8, P11, P13], \textit{``is multi-faceted''} [P13], \textit{``involves objectively learning about a domain that requires more time''} [P11, P18] and \textit{``more unfamiliar and technical terminology''} [P13].

Furthermore, these two search tasks, although both exploratory, were perceived to possess different attributes. Overall, the Politics task was found to be more subjective, required more high level information and belonged to the Learn category of exploratory search tasks \cite{marchionini06}. This task was also found to be a precision oriented task as exploration was done mostly at a higher level and learning a few accurate facts about how each president functions locally or globally could suffice for comparison.
The History task, on the other hand, was seen as more objective and was characterized as more of a finding task that involves more detailed information and fact retrieval, closer to the Investigate category of exploratory search task \cite{marchionini06}. This task also seemed to share attributes of recall oriented tasks where a higher number of relevant facts need to be retrieved to satisfy the search task.
\vspace{-1.6mm}
\begin{myquote}{0.2in}
    \textit{``For the Politics task I thought that I had to learn something, whereas for the other one I didn't feel I need to learn anything. 
    %And it could be my lack of knowledge on the subject of Politics that made it feel like I know nothing about this. 
    Like in order to make any reasonable statement I will have to actually learn something about these countries.''} [P8]
\end{myquote}
The second theme that arose from our qualitative analysis explored how knowledge graphs generated at different levels of quality, as measured by precision and recall, were perceived by participants performing exploratory search tasks. To our surprise, participants did not notice any significant quality differences between the knowledge graphs they interacted with across the two search tasks and they were not able to identify the automatically generated ones when were specifically asked to do so.
\begin{myquote}{0.2in}
    \textit{I think if you come across contradictory knowledge when you're not confident about your prior knowledge then I would maybe try to accept both of them and try to justify them in my mind.} [P5]
\end{myquote}

The final theme from our qualitative interviews explored the factors that may help or hinder noticing of errors in automatically extracted information and contrasted the impact of these errors between lookup and exploratory search tasks. We found that the intent of the user performing the task (i.e., information seeking versus validating information), their confidence in the task (i.e., their prior knowledge of the topic as well as their language competency) and different types of cognitive biases impact the likelihood of noticing errors.
\begin{myquote}{0.2in}
%    \textit{Now I can see that mostly when I reading sentences I look at keywords only. Especially when it's not written in my first language. And sometimes it feels like all English sentences should make sense, which is not the case in my first language, Persian. I do validate sentences as I read them in my first language!}[P13]
\textit{ I  think there are multiple factors to consider. One thing is about my confidence in some language. When I read sentences in English, I don't question the validity as often as I do when I read text in my first language. 
% And I simply assume the sentences must be accurate. 
So I'm more focused on understanding what the sentence is trying to say and not so much on spotting potential grammar issues, typos or inconsistent information. [...]
And for more technical texts it's a mix of unfamiliarity and lack of confidence in my own knowledge of the domain as well as a higher level of trust in the validity of information that makes me accept what I read as facts.} [P13]
\end{myquote}
Alongside participant comments, data from our field notes and observations indicated that the impact of poor quality of extracted information is higher for lookup and factoid question answering tasks than in the exploratory search tasks. The sensemaking aspect of exploratory search tasks coupled with the time willing to be spent in these tasks seem to play a role in mitigating the impact of errors to some extent.

\begin{myquote}{0.2in}
    \textit{``I'm more likely to notice errors when I dig deeper, I'm investigating further and when I'm inclined to read the articles text. These are the case in the Complex Task.''} [P9]\\
    \textit{``[for a Complex task] I'm trying to get a big picture or form an idea, whereas here [in Simple task] I'm looking for specific information.
    It's like a `ray of light' and a small error like that would have completely deflected it!
    Where as for the complex task I was `shining a lot of light` so small errors could cast a little shadow but then you'll get lots of other beams of light! ''} [P8]
\end{myquote}
\vspace{-1.05em}






==> sec.RelatedWork.tex <==
\section{Related Work}
\textcolor{red}{As noted in the introduction, our primary interest in this work is to develop an understanding of how errors in information extraction impact exploratory search.  In this section, we provide background in IR research on the effect of error on information seeking and examine past research in supporting exploratory search.}

\subsection{Error Effects in Information Seeking}
It is often assumed if an evaluation measure coupled with a test collection reveals that system A provides higher quality output than system B, then the user will both prefer system A and that system A will more effectively support the user's information seeking task \cite{Allan05, vakkari12}.  However, the IR research on this topic indicates that the relationship between output quality and system efficacy is not clear.

In document retrieval, there is a long history of research that examines how human search performance varies with system effectiveness \cite{hersh2000, turpin01, Allan05, turpin06, church90, almaskari08good, smith08, sanderson10, smucker08, wang15}. The broader goal of this line of work is to understand when system effectiveness improvements are meaningful or useful in improving users' information seeking abilities in practice. 
These studies, however, have resulted in contradictory findings. Early studies suggest that ``better'' systems, as measured by system oriented metrics such as precision and recall, do not necessarily translate into better task performance \cite{hersh2000, turpin01, hersh02, turpin06, smith08}.  More recent work has detected potential correlations between various system effectiveness metrics and human preferences \cite{almaskari08good, sanderson10} and between precision and user performance \cite{smucker10}. 

Even if one gives credence to more recent work relating  effectiveness to user preference and user performance, the reason for inconsistent effects of system performance on human performance in past work is unclear.  Differences could lie in the definition of `relevance' and how it is used as a basis for evaluation of document retrieval systems \cite{doyle63, swanson77, saracevic}; they could also lie in the discrepancies between the metrics used for evaluation (e.g., MAP vs P@10) and the type of task the user performs (e.g., recall-based or complex information seeking) \cite{turpin06}; sample size may provide increased power to discriminate effects \cite{almaskari08good, sanderson10}; or, finally, differences could be a result of the lack of UI support for meaningful user interaction with the retrieved results \cite{lin08, smith08, turpin01}. Hersh et al.~\cite{hersh02} also found that while precision and recall weren't associated with success in medical QA tasks, other factors including experience of the searcher and cognitive abilities in spatial visualization were correlated with the ability to answer questions correctly.

% For example, some past work has demonstrated that searchers were able to maintain the same level of performance regardless of the system effectiveness by working harder, for example,  by issuing more queries \cite{smith08}, reading more documents \cite{turpin01} or browsing \cite{lin08} to compensate for poor search results. 
%Swanson \cite{swanson77} was one of the early critics of evaluating retrieval systems based on their ability to select relevant documents. Doyle \cite{doyle63} also argues that retrieval systems should be evaluated on the basis of their exploratory capabilities since it is essentially impossible to measure their ability to deliver documents relevant to an actual information need. 
% Finally, Vakkari and Huuskonen \cite{vakkari12} argue that, most IR evaluation efforts has focused on system output rather than outcomes, where outputs are the products delivered by a system and outcomes are the benefits the system produces for its users. 
% %(Rossi, Lipsey, \& Freeman, 2004).

Possibly due to the ambiguous link between system performance and effectiveness, there have been calls to extend evaluation of IR systems from an analysis of the output of the system to the outcome of the search task \cite{kelly09, vakkari12}.  Furthermore, there is also an evolving drive toward evaluations of how effectively IR systems support complex, evolving, long term information seeking goals, such as learning and exploration \cite{swirl2018}. % This support requires advances in algorithms, interfaces and evaluation methods that support these goals. 
\vspace{-1mm}
% investigated  the  effects  of  combining  a  knowledge  graph  with textual  documents.   Their  goal,  like  ours,  was  to  understand user behaviour with respect to different search tasks. They argue that a hybrid approach that combines the coherent content of text with the organized structure of graphs may better support information finding and sense making. They  conclude  that  utilizing  graphs  of  concepts  and  relationships which are derived from documents can be effective for finding relevant information when the information need is  well  defined.   Their  findings  also  demonstrate  that  providing  meaningful  relations  that  explain  how  different  entities of a domain are connected are crucial for supporting more complex search task.  Our work broadens this work by looking specifically at the contrast between hierarchical representations  (e.g.   trees)  and  network  representations  (e.g. knowledge graphs).

% This area of related research also involves understanding cognitive aspects of users that are relevant to their information seeking and can influence their interactions with retrieved information and how they assess this information. Some examples include investigating how cognitive biases can result in irrational search behavior and influence searchers' relevance judgement of information \cite{white13} or how the idea of bounded rationality impacts the way information seekers optimize their information processing efforts even at the cost of achieving a sub-optimal outcome \cite{pirolli05}.
% biases can be observed in information retrieval in situations where searchers seek or are presented with information that significantly deviates from the truth \cite{white13}. 
% In fact, information foraging theory \cite{pirolli05}, inspired by the idea of bounded rationality and satisficing, states that information seekers, will choose behaviors that optimize the utility of information gained as a function of interaction cost.

% Finally, developing solutions to support users' exploratory search tasks also includes significant challenges in evaluation. The recent SWIRL Workshop \cite{swirl2018} has identified the most relevant research questions to be addressed in order to develop new evaluation models that are suited for complex and exploratory information seeking. A major step towards this goal is to design and study characteristics of search tasks that elicit exploratory behavior and enable means to study searchers performing these tasks, their outcomes and behaviors. 
% The literature \cite{marchionini06, bystrom95, bystrom05, kules08, li_belkin08, wildemuth12} suggests a number of desirable characteristics for exploratory search (see Section 3 for details).

% Synthesizing past research, we see ambiguity in the effect of errors in the domain of information retrieval \cite{}, and an increasing focus on outcome versus output centric assessment \cite{}. Coupled with this, we note that exploratory search tasks require systems that support browsing, and, within information retrieval, this has given rise to systems that retrieve and present information to users in formats that support browsing \cite{}.  However, one thing that seems absent from past research is any assessment of the effect of information extraction errors on exploratory search interfaces: \fixme{many assessments of exploratory search interfaces leverage human-generated information representations \cite{}}.  While we concur that systems would ideally have perfect precision and recall, in the near term it seems unlikely that computational information extraction will be perfected.  In this work, we pose specifically this question, examining the effect of information extraction errors on interfaces that support exploratory search.\textcolor{blue}{TODO: add the IBM paper for IE errors.}

\begin{comment}
\textcolor{blue}{These are the main areas of related work I think we need to discuss:}
\begin{enumerate}
    \item Relationship between Systems' Effectiveness and Users' Search Performance 
        \begin{itemize}
            \item Variations in Relevance Judgement does not affect System's relative ranking
            \item IR systems poor performance does not necessarily mean bad search performance -> users can recover and still do well
        \end{itemize}
        \item Supporting Exploratory Search Tasks
            \begin{itemize}
                \item The need for alternative representations and paradigms of interaction ..
                \item Designing Exploratory Search Tasks (that enables Evaluation of systems supporting Exploratory Search Tasks)
            \end{itemize}
\end{enumerate}
\end{comment}

\subsection{Designing for Exploratory Search}
While there has been research on understanding complex and exploratory search (see \cite{white09, wilson10} for a survey), there are many open questions when it comes to the design and evaluation of IR systems that provide tailored and adaptive support for long-term search needs.
% as well as overcoming challenges in evaluating how well such systems support searchers in learning and discovery. 
We have identified three areas of past research that explore support for users with more complex, exploratory search tasks.
First, there has been a growing body of work in the IR community that aims to deliver ``information'' and not documents. Within this body of work, Open Information Extraction (Open IE) \cite{banko07} techniques have been widely applied to extract semantic information from the text of documents to support a variety of down stream applications such as question answering or to populate knowledge bases (see \cite{niklaus2018survey} for a recent survey of these systems).
% Information Extraction (IE), Question Answering (QA) and Summarization all generate a focused response to a user’s information need in the form of entities, sentences or text snippets. 
% These  solutions  focus  on  retrieving  information  as  opposed  to  documents  to  address  the  user’s information need.

\bs{SigIR-RW Section ``Organizing Search Results" can be merged here.}
The second area focuses on investigating ways that search systems can represent and provide the extracted information to help searchers in evaluating and contextualizing search results. 
Information seekers express a need for tools that organize search
results into meaningful constructs in order to support sensemaking and navigation \cite{hearst06, marchionini06}. As a result, \emph{spatial models} \cite{novick01} such as hierarchies and networks have been used to organize information and support sensemaking \cite{ltifi2009}.
A taxonomy of these
techniques for organizing search results was proposed by Wilson et al. \cite{wilson10}. 
% Capra et al.  [9], in their study on the relationships between search tasks, information architecture and interaction style, note, among other observations, that  users  gain  benefits  from  support  for  facets and  topic organization implemented in a flexible style.
Within this space of techniques for the organization of search results, researchers  have performed evaluations of representations including concept maps \cite{amadieu10,amadieu14, carnot03}, hierarchies (e.g. \cite{capra07, norman88, ducheneaut01}) and networks (\cite{sarrafzadeh14}). 
% Other recent work in search results representation focuses on a single visualization (e.g.  concept maps) that seeks to represent both hierarchies and networks () to support information seeking and finding.  
More recently Sarrafzadeh et al. \cite{sarrafzadeh16, sarrafzadeh17} designed search interfaces looking specifically at the contrast between hierarchical and network representations.  

Finally, developing solutions to support users' exploratory search tasks also includes significant challenges in evaluation. The recent SWIRL Workshop \cite{swirl2018} has identified the most relevant research questions to be addressed in order to develop new evaluation models that are suited for complex and exploratory information seeking. A major step towards this goal is to design and study characteristics of search tasks that elicit exploratory behavior.  
\bs{SigIR-RW Section ``Understanding web search" can be merged here.}
These studies, in turn, provide data on searchers performing these tasks, specifically focused on task outcomes and searcher behaviors. 
Designing tasks for exploratory search studies can be especially difficult since inducing exploratory style search requires searcher to individually interpret the tasks, results, and their relevance ~\cite{kules08shneiderman} which is at odds with maintaining some level of experimental control and consistency~\cite{kules08}.
% Designing exploratory search tasks is an important but challenging requirement for successfully evaluating exploratory search interfaces. 
% %When creating any type of search task, there is a challenge of creating a realistic, representative task. When creating exploratory search tasks, there is an additional burden of actually inducing an exploratory search \cite{kules08}.
% As Kules and Capra \cite{kules08} have pointed out, ``designing tasks for studies of exploratory search can be especially difficult due to the goal of inducing an exploratory (rather than directed) style search, wherein searchers will individually interpret the tasks, their relevance, and the results \cite{kules08shneiderman} - while maintaining some level of experimental control''.
% % This high level goal of doing an exploratory search drives how users interpret their tasks, their relevance and their results \cite{kules08shneiderman}.
The literature \cite{marchionini06, bystrom95, bystrom05, kules08, li_belkin08, wildemuth12} suggests a number of desirable characteristics for exploratory search.  
% As well, given that search tasks can vary among many dimensions (e.g. their complexity, structure and granularity), 
As Wildemuth and Freund \cite{wildemuth12} note, it is crucial to construct tasks having particular attributes, knowing that our study findings can then be generalized to all search tasks having those attributes. 

\textcolor{red}{Our primary interest is in how errors in IE impact end-user performance and effort in exploratory search.}  
Within the broad domain of the impact of error in IE, we were able to identify only one work by Chu-Carrol and Prager \cite{chu07} that examined how user performance degrades in the face of imperfect named entity and relation extraction. Their experimental results demonstrated that significant document retrieval gain can be achieved when state-of-the-art IE systems are used and that recall has more significant impact on document retrieval performance than precision when adopting the MAP metric.  Their results focus on assessment of document retrieval, not on assessment of support for exploratory search.

\bs{Both the following paragraph and the first subsection of RW (Error Effects in Information Seeking) are only related to part II while the rest of this RW and RW from SigIR can be related to both parts. Need a new structure for the RW section?}

Synthesizing past research, we see ambiguity in the effect of errors in the domain of information retrieval, and an increasing focus on outcome versus output centric assessment. Coupled with this, we note that exploratory search tasks require systems that support browsing, and, within information retrieval, this has given rise to systems that retrieve and present information to users in formats that support browsing.  However, absent from past research is any assessment of the effect of information extraction errors on exploratory search interfaces.  While we concur that systems would ideally have perfect precision and recall, in the near term it seems unlikely that computational information extraction will be perfected, further motivating exploration of the effect of information extraction errors on interfaces that support exploratory search.

\begin{comment}
The literature suggests a number of desirable characteristics for exploratory search. Marchionini (2006) lists exploratory tasks,  characterizing  them  as  either  learning-oriented  or 
investigative.  This  suggests  that  the  high-level  scenario 
should   be   described   so   that   it   involves   learning   or investigation.   Kuhlthau   (1991)   describes   six   stages of search  and  predicts  various  types  of  searcher  interaction. 
Early stages are characterized by uncertainty. 

Task  complexity  refers  to  the  degree  of  pre-determinability of  task  performance  (Bystrom  and  Jarvelin,  1995).  Some 
tasks  are  well  established  and  understood  (known), while others   are   more   unique   and   less   understood   (genuine decision  tasks).  Problem  structure,  task  complexity and prior   knowledge   have   an   interconnecting   impact   when searching.   ``The   more   complex   the   task,   the   more   ill- structured it is, and the less prior knowledge the actor has.'' (Vakkari 1999).  

Borlund (2000) advises that simulated situations include: ``i. A situation which the test persons can relate to and in which they  can  identify  themselves;  ii.  A  situation  that the  test  
persons  find  topically  interesting,  and;  iii. A  situation  that provides  enough  imaginative  context  in  order  for  the  test 
persons to be able to relate and apply the situation.'' 

Kules  \&  Shneiderman  (2003)  used  four  simulated  work
tasks   for   journalists   constructed   around   an   exploratory search  task  to  evaluate  a  faceted  web  search  interface, 
drawing  on  Yee  et  al.  (2003),  which  included  open-ended tasks that were constructed with similar objectives. 

Bystrom and Hansen (2005) characterized tasks that are important to interactive IR  researchers as  occurring  at  three  levels: information-intensive work   tasks,   information   seeking   tasks,   and information search tasks. 

In 2008, two different approaches were proposed to develop search tasks that can support experimental research and system evaluation in more realistic contexts.
Kules and Capra \cite{kules08} designed a template for developing exploratory tasks mimicking a 'paper writing for a class' scenario that is familiar to student participants. 
Taking a different approach, Li and Belkin \cite{li_belkin08} identified and developed a taxonomy of the attributes of tasks (including both work tasks and search tasks). The taxonomy includes both generic facets of tasks (e.g. source, time-related attributes, and goals) and common attributes (e.g. complexity, difficulty and urgency). As researchers develop search tasks, they can use this taxonomy to specify the task attributes of interest for a particular study.

Wildemuth and Freund \cite{wildemuth12} conducted a large scale systematic review of past studies and the employed search tasks and identified a set of task characteristics associated with exploratory search tasks: 
exploratory  search  tasks  focus  on learning  and  investigative search  goals;  they  are  general (rather than specific), open-ended, and often target multiple items/documents;    they    involve    uncertainty    and    are motivated by ill-defined or ill-structured problems; they are dynamic  and  evolve  over  time;  they  are  multi-faceted  and may be   procedurally complex; and they are often accompanied  by  other  information  or  cognitive behaviors, such  as  sensemaking.

\end{comment}
